Automatically finding atomic regions for fixing bugs in Concurrent programs

This paper presents a technique for automatically constructing a fix for buggy concurrent programs: given a concurrent program that does not satisfy user-provided assertions, we infer atomic blocks that fix the program. An atomic block protects a piece of code and ensures that it runs without interruption from other threads. Our technique uses a verification tool as a subroutine to find the smallest atomic regions that remove all bugs in a given program. Keeping the atomic regions small allows for maximum concurrency. We have implemented our approach in a tool called AtomicInf. A user of AtomicInf can choose between strong and weak atomicity semantics for the inferred fix. While the former is simpler to find, the latter provides more information about the bugs that got fixed. We ran AtomicInf on several benchmarks and came up with the smallest and the most precise atomic regions in all of them. We implemented an earlier technique to our setting and observed that AtomicInf is 1.7 times faster on an average as compared to an earlier approach.

==> background.tex <==
\section{Background}
Background details here


==> blocks.tex <==



\Omit{For the example shown in \figref{banking} the tool found a solution which is smaller
than the one given in \figref{bankingfix}. For the assertion to be satisfied, we do
not need context switch to be disabled at line \ref{csallowed} as shown in
\figref{toolfix}. Hence, the proposed
solution consists of two regions (line \ref{atom1start}-\ref{atom1end}) and (line
\ref{atom2start}-\ref{atom2end}). Our tool proposes the smallest solution which is
sufficient to satisfy the assertion given.

If \TT{thread2} in \figref{banking} is replaced by the one shown in 
\figref{bankingcorpus}, then the tool indeed proposes a single strong atomic region in \TT{transfer}
(line (\ref{atom1start}-\ref{atom2end}) in \figref{toolfix}).

\begin{figure}
\begin{tabular}{p{5cm}}
\begin{scriptsize}
\begin{Verbatim}[numbers=left,commandchars=*\[\]]
int transfer(Account* src,Account* dst,int amount)
{
  satomic
   {
      if(src.amount>=amount) *label[atom1start]
      {
        int temp = src.amount;
        temp = temp - amount;
        src.amount = temp; *label[atom1end]
   --> *label[csallowed]     
        temp = dst.amount; *label[atom2start]
        temp = temp + amount; *label[atom2end]
        dst.amount = temp
        return 1;
      }
   }
      return 0;
}
\end{Verbatim}
\end{scriptsize}
\end{tabular}
\caption{strong atomicity fix for program in fig. \ref{Fi:banking} by our tool }
\label{Fi:toolfix}
\end{figure}


\begin{figure}
\begin{scriptsize}
\begin{Verbatim}[numbers=left,commandchars=&\[\]]
void thread2()
{
   int temp=0;
   satomic{
	   temp = acc1.account;
           temp += acc2.account;
           temp += acc3.account;
           assert(temp == 600);
   }
}

\end{Verbatim}
\end{scriptsize}
\caption{Corpus of the bank must be constant at all times}
\label{Fi:bankingcorpus}
\end{figure}

} %end of Omit


